Conversational Education at Scale: A Multi-LLM Agent Workflow for Procedural Learning and Pedagogic Quality Assessment

Large language models (LLMs) have advanced virtual educators and learners, bridging NLP with AI4Education. Existing work often lacks scalability and fails to leverage diverse, large-scale course content, with limited frameworks for assessing pedagogic quality. To this end, we propose WikiHowAgent, a multi-agent workflow leveraging LLMs to simulate interactive teaching-learning conversations. It integrates teacher and learner agents, an interaction manager, and an evaluator to facilitate procedural learning and assess pedagogic quality. We introduce a dataset of 114,296 teacher-learner conversations grounded in 14,287 tutorials across 17 domains and 727 topics. Our evaluation protocol combines computational and rubric-based metrics with human judgment alignment. Results demonstrate the workflow's effectiveness in diverse setups, offering insights into LLM capabilities across domains. Our datasets and implementations are fully open-sourced.

==> figure/all_model_performance_across_domain.tex <==
\begin{figure*}[!htb]
  \centering
  % First row: legend
  \begin{subfigure}[b]{\textwidth}
    \includegraphics[trim=3cm 27.76cm 0cm 2cm, clip, width=\textwidth]{figure/T-openchat_L-openchat_E-openchat_11297606_corrected_legend.png}
    % \caption{legend}
  \end{subfigure}
  % Second row
  \begin{subfigure}[b]{0.22\textwidth}
    \includegraphics[width=\textwidth]{figure/T-deepseek-llm_L-deepseek-llm_E-deepseek-llm_11246257_corrected.png}
    \caption{deepseek}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.22\textwidth}
    \includegraphics[width=\textwidth]{figure/T-qwen2_L-qwen2_E-qwen2_11236934_corrected.png}
    \caption{qwen2}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.22\textwidth}
    \includegraphics[width=\textwidth]{figure/T-gemma_L-gemma_E-gemma_11269574_corrected.png}
    \caption{gemma}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.22\textwidth}
    \includegraphics[width=\textwidth]{figure/T-olmo2_L-olmo2_E-olmo2_11370185_corrected.png}
    \caption{olmo2}
  \end{subfigure}
    % Third row
    \begin{subfigure}[b]{0.22\textwidth}
        \includegraphics[width=\textwidth]{figure/T-openchat_L-openchat_E-openchat_11297606_corrected.png}
        \caption{openchat}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.22\textwidth}
        \includegraphics[width=\textwidth]{figure/T-llama3_L-llama3_E-llama3_11232754_corrected.png}
        \caption{llama3}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.22\textwidth}
        \includegraphics[width=\textwidth]{figure/T-phi4_L-phi4_E-phi4_11269383_corrected.png}
        \caption{phi4}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.22\textwidth}
        % \includegraphics[width=\textwidth]{radar8.png}
        \caption{gpt4}
    \end{subfigure}
  \caption{Multiple rubric evaluation scores over various domains across varying LLMs.}
\end{figure*}

==> table/article_per_domain_v2.tex <==
\begin{table}[h!]
\centering
\scriptsize
\resizebox{\textwidth}{!}{
\begin{tabular}{@{}clclclclclc@{}}
\toprule
\textbf{ID} & \textbf{Domain}         & \textbf{\#Article} & \textbf{} & \textbf{ID} & \textbf{Domain}         & \textbf{\#Article} & \textbf{} & \textbf{ID} & \textbf{Domain}   & \textbf{\#Article} \\ 
% \cmidrule(lr){1-3}\cmidrule(lr){5-7} \cmidrule(lr){9-11}
\midrule
1            & Automobiles \& Vehicles & 166                &           & 
7            & Family \& Parenting     & 150                &           & 
13           & Pets \& Animals   & 131                \\
2            & Business \& Finance     & 98                 &           & 
8            & Food \& Cooking         & 127                &           & 
14           & Relationships     & 368                \\
3            & Career \& Workplace     & 139                &           & 
9            & Health                  & 363                &           & 
15           & Self-Improvement  & 222                \\
4            & Culture \& Lifestyle    & 197                &           & 
10           & Hobbies \& Leisure      & 306                &           & 
16           & Technology        & 227                \\
5            & Education               & 296                &           & 
11           & Home \& Garden          & 266                &           & 
17           & Travel \& Leisure & 61                 \\
6            & Entertainment           & 209                &           & 
12           & Personal Care \& Beauty & 358                &           &              &                   &                    \\ \bottomrule
\end{tabular}
}
\caption{Number of WikiHow articles across 17 domains.}\label{tab:article_per_domain}
\end{table}

==> table/article_per_topic.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table*}[htb!]
\centering
\tiny
\resizebox{\textwidth}{!}{
\begin{tabular}{@{}llcllcllc@{}}
\toprule
\textbf{No.}   & \textbf{Topic}               & \multicolumn{1}{r}{\textbf{\#Article}} & \textbf{No.}   & \textbf{Topic}              & \multicolumn{1}{r}{\textbf{\#Article}} & \textbf{No.}   & \textbf{Topic}                     & \multicolumn{1}{r}{\textbf{\#Article}} \\ \midrule
\textbf{{[}1{]}}  & Sports-and-Fitness           & 98                                 & \textbf{{[}28{]}} & Work-World                  & 63                                 & \textbf{{[}55{]}} & Artwork                            & 29                                 \\
\textbf{{[}2{]}}  & Garden-Pests-and-Weeds       & 90                                 & \textbf{{[}29{]}} & Putty-Dough-and-Slime       & 59                                 & \textbf{{[}56{]}} & Weight-Loss-Goals                  & 29                                 \\
\textbf{{[}3{]}}  & Cars-\&-Other-Vehicles       & 88                                 & \textbf{{[}30{]}} & Crafts                      & 58                                 & \textbf{{[}57{]}} & Computers                          & 28                                 \\
\textbf{{[}4{]}}  & Hobbies-and-Crafts           & 87                                 & \textbf{{[}31{]}} & Philosophy-and-Religion     & 51                                 & \textbf{{[}58{]}} & Books                              & 28                                 \\
\textbf{{[}5{]}}  & Health                       & 85                                 & \textbf{{[}32{]}} & Communication-Skills        & 51                                 & \textbf{{[}59{]}} & Men's-Health                       & 28                                 \\
\textbf{{[}6{]}}  & Home-and-Garden              & 85                                 & \textbf{{[}33{]}} & Drawing                     & 49                                 & \textbf{{[}60{]}} & Using-PDF-Files                    & 26                                 \\
\textbf{{[}7{]}}  & Education-\&-Communication   & 81                                 & \textbf{{[}34{]}} & Driving-Basics              & 47                                 & \textbf{{[}61{]}} & Personal-Care                      & 25                                 \\
\textbf{{[}8{]}}  & Personal-Care-and-Style      & 81                                 & \textbf{{[}35{]}} & Love                        & 46                                 & \textbf{{[}62{]}} & Ant-and-Termite-Control            & 25                                 \\
\textbf{{[}9{]}}  & Education-and-Communications & 81                                 & \textbf{{[}36{]}} & Studying                    & 45                                 & \textbf{{[}63{]}} & House-Training-Cats                & 21                                 \\
\textbf{{[}10{]}} & Food-and-Entertaining        & 80                                 & \textbf{{[}37{]}} & Fashion                     & 44                                 & \textbf{{[}64{]}} & Women's-Health                     & 21                                 \\
\textbf{{[}11{]}} & Computers-and-Electronics    & 80                                 & \textbf{{[}38{]}} & Curly-Hair                  & 44                                 & \textbf{{[}65{]}} & Air-Travel                         & 20                                 \\
\textbf{{[}12{]}} & Youth                        & 79                                 & \textbf{{[}39{]}} & Calculating-Volume-and-Area & 42                                 & \textbf{{[}66{]}} & Clogged-Pores-(Comedones)          & 20                                 \\
\textbf{{[}13{]}} & Games                        & 79                                 & \textbf{{[}40{]}} & Mental-Health               & 42                                 & \textbf{{[}67{]}} & Technology-Hacks                   & 19                                 \\
\textbf{{[}14{]}} & Love-and-Romance             & 77                                 & \textbf{{[}41{]}} & Travel                      & 40                                 & \textbf{{[}68{]}} & Death-Funerals-and-Bereavement     & 17                                 \\
\textbf{{[}15{]}} & Personal-Development         & 76                                 & \textbf{{[}42{]}} & Phone-Skills                & 39                                 & \textbf{{[}69{]}} & Turkey-Dishes                      & 17                                 \\
\textbf{{[}16{]}} & Pets-and-Animals             & 74                                 & \textbf{{[}43{]}} & Handling-Rejection          & 38                                 & \textbf{{[}70{]}} & Egg-Basics                         & 16                                 \\
\textbf{{[}17{]}} & Android                      & 74                                 & \textbf{{[}44{]}} & Job-Search                  & 36                                 & \textbf{{[}71{]}} & School-Leadership                  & 16                                 \\
\textbf{{[}18{]}} & Relationship-Issues          & 73                                 & \textbf{{[}45{]}} & Dogs                        & 36                                 & \textbf{{[}72{]}} & Guitar-Chords-and-Songs            & 15                                 \\
\textbf{{[}19{]}} & Hair-Care                    & 73                                 & \textbf{{[}46{]}} & Business-Writing            & 36                                 & \textbf{{[}73{]}} & Cakes                              & 14                                 \\
\textbf{{[}20{]}} & Dating                       & 71                                 & \textbf{{[}47{]}} & Abdominal-Exercises         & 35                                 & \textbf{{[}74{]}} & Positive-and-Reflective-Lifestyles & 13                                 \\
\textbf{{[}21{]}} & Family-Life                  & 71                                 & \textbf{{[}48{]}} & Birthdays                   & 34                                 & \textbf{{[}75{]}} & Motivation-to-Exercise             & 13                                 \\
\textbf{{[}22{]}} & Finance-and-Business         & 69                                 & \textbf{{[}49{]}} & Movies                      & 33                                 & \textbf{{[}76{]}} & Reproductive-Health                & 12                                 \\
\textbf{{[}23{]}} & Arts-and-Entertainment       & 69                                 & \textbf{{[}50{]}} & Married-Life                & 32                                 & \textbf{{[}77{]}} & Singing                            & 9                                  \\
\textbf{{[}24{]}} & Relationships                & 69                                 & \textbf{{[}51{]}} & Astrology                   & 32                                 & \textbf{{[}78{]}} & Skin-Tone                          & 6                                  \\
\textbf{{[}25{]}} & Cleaning-Metals              & 66                                 & \textbf{{[}52{]}} & School-Stuff                & 31                                 & \textbf{{[}79{]}} & Better-Writing                     & 5                                  \\
\textbf{{[}26{]}} & Personal-Hygiene             & 65                                 & \textbf{{[}53{]}} & Motorcycles                 & 31                                 & \textbf{{[}80{]}} & Meetings                           & 4                                  \\
\textbf{{[}27{]}} & Holidays-and-Traditions      & 63                                 & \textbf{{[}54{]}} & Checks-and-Checkbooks       & 29                                 & \textbf{{[}81{]}} & Official-Travel-Documentation      & 1                                  \\ \bottomrule
\end{tabular}
}
\caption{Frequency of topics.}\label{tab:topics}
\end{table*}

==> table/rubrix_small_tables.tex <==
\begin{table}[h!]
    \centering
    \resizebox{\columnwidth}{!}{%
        \begin{tabular}{|c|c|c|}
            \hline
            \textbf{Criteria} & \textbf{Description} & \textbf{Score} \\ \hline
            1. Relevance & How relevant is the generated article to the input query? & 0-5 \\ \hline
            2. Coherence & Is the article coherent and logically structured? & 0-5 \\ \hline
            3. Informativeness & Does the article provide useful and informative content? & 0-5 \\ \hline
            4. Clarity & Is the language clear and easy to understand? & 0-5 \\ \hline
            5. Engagement & Is the article engaging and interesting to read? & 0-5 \\ \hline
        \end{tabular}%
    }
    \caption{Detailed rubric for evaluating the generated articles.}
    \label{tab:rubric}
\end{table}
\begin{table}[h!]
    \centering
    \resizebox{\columnwidth}{!}{%
        \begin{tabular}{|c|c|}
            \hline
            \textbf{Score} & \textbf{Description} \\ \hline
            0 & No relevance or coherence \\ \hline
            1 & Very low relevance, coherence, and informativeness \\ \hline
            2 & Low relevance, coherence, and informativeness \\ \hline
            3 & Moderate relevance, coherence, and informativeness \\ \hline
            4 & High relevance, coherence, and informativeness \\ \hline
            5 & Excellent relevance, coherence, and informativeness \\ \hline
        \end{tabular}%
    }
    \caption{Scoring system for the evaluation rubric.}
    \label{tab:score}
\end{table}
